Similarity-Aware Skill Reproduction based on Multi-Representational Learning from Demonstration

Learning from Demonstration (LfD) algorithms enable humans to teach new skills to robots through demonstrations. The learned skills can be robustly reproduced from the identical or near boundary conditions (e.g., initial point). However, when generalizing a learned skill over boundary conditions with higher variance, the similarity of the reproductions changes from one boundary condition to another, and a single LfD representation cannot preserve a consistent similarity across a generalization region. We propose a novel similarity-aware framework including multiple LfD representations and a similarity metric that can improve skill generalization by finding reproductions with the highest similarity values for a given boundary condition. Given a demonstration of the skill, our framework constructs a similarity region around a point of interest (e.g., initial point) by evaluating individual LfD representations using the similarity metric. Any point within this volume corresponds to a representation that reproduces the skill with the greatest similarity. We validate our multi-representational framework in three simulated and four sets of real-world experiments using a physical 6-DOF robot. We also evaluate 11 different similarity metrics and categorize them according to their biases in 286 simulated experiments.

==> extra.tex <==
As robots become increasingly present in the world, they are expected to be able to learn, reproduce, and generalize new skills effortlessly and robustly. One of the most intuitive ways to teach skills to robots is through Learning from Demonstration (LfD) \cite{survey}. LfD enables humans to teach new primitive skills (e.g., reaching) to robots only by providing examples, bypassing the need for manual programming of the movements into the system. Several LfD algorithms with various representations have been developed and evaluated~\cite{ravichandar2020recent}. 
%\reza{Some of these representations encode a skill from a single demonstration. Although providing a single demonstration reduces the effort of the end-user, however, generalizing from a single demonstration can result in reproductions that conflict with what the user intended. To capture a more generalized and flexible skill model, on the other hand, some representations rely on a set of diverse human provided demonstrations. Potentially, each demonstration in the set represents the execution of the skill under a specific condition or constraint. It should be noted that a set of similar demonstrations implies a small variance of the movement over time. Multi demonstration LfD algorithms try to capture the variance of the demonstrated skill through different modeling representations that could be categorized into four groups: statistical (GMM, TPGMM), dynamical systems (CorrDMP, SEDS), geometric (TLGC), and probabilistic (CLAMP, ProMP). These representations provide different ways of modeling and generalizing a skill with the goal of capturing the main characteristics of the skill as intended by the user.
%In this paper, we propose a meta learning framework that uses a set of LfD representations in order to generalize a skill with better similarity under different circumstances. Given a single demonstration, our framework builds a similarity map in the generalization space (i.e. a space around the initial or end-point of the demonstration) and uses the representation that reproduces the skill while maximizing the similarity between the demonstration and the reproduction. To address this issue, we propose a Meta-Learning from Demonstration (MLfD) algorithm that generates a robust generalization region for a given demonstration. The algorithm first generates a meshgrid around a user-selected desired point (e.g., initial, final, via-point). It then uses an ensemble of LfD representations and a similarity metric to calculate similarity values of the generated meshgrid for each representation. The constructed map represents the similarity between the demonstration and the reproductions of the skill at each point. Given a new point (e.g., initial), MLfD selects the optimal representation to reproduce the skill with maximum similarity. In addition, given a similarity percentage, the algorithm returns a region within which the task can be generalized robustly. The region is constructed by unifying the obtained similarity maps through interpolation. 
%}

Some of these representations encode a skill from a single demonstration~\cite{LTE,JA,IjspeertDMP2013}. Providing a single demonstration reduces the effort of the end-user, but generalizing from a single demonstration can result in reproductions that conflict with user intentions. To capture a more generalized and flexible skill model, some representations rely on a set of diverse human provided demonstrations~\cite{GMMcalinon2007,LASA,TLGC,ProMP,CorrDMP}. Multi demonstration LfD algorithms try to capture the spatial or temporal variance of the demonstrated skill through different modeling representations (e.g., probabilistic~\cite{ProMP}, geometric~\cite{TLGC}, statistical~\cite{TPGMMcalinon2016}, and dynamical systems~\cite{LASA, IjspeertDMP2013}). These representations provide different ways of modeling and generalizing a skill with the goal of capturing the main characteristics of the skill as intended by the user. However, it has been shown that providing multiple demonstrations of a skill that are diverse enough, cover the demonstration space, and satisfy all the skill constraints is neither intuitive nor convenient for end-users~\cite{GT_dataset}.

%that could be categorized into four groups: statistical (GMM \cite{GMMcalinon2007}, TPGMM \cite{TPGMMcalinon2016}), dynamical systems (CorrDMP \cite{CorrDMP}, SEDS \cite{LASA}), geometric (TLGC \cite{TLGC}), and probabilistic (ProMP \cite{ProMP})

In this paper, we propose a Meta-Learning from Demonstration (Meta-LfD) framework that consists of a set of various single-demonstration LfD representations together with a similarity metric. Given a single demonstration of a skill, Meta-LfD  evaluates the outcomes of different representations using the similarity metric and provides the user with (a) an optimal (most similar) reproduction of the skill for a given new condition including initial, final, or via-points, and (b) a similarity region, which contains information on each representation's ability to generalize over different points in space. Our framework offers better generalization capabilities with respect to each individual (single-demonstration) representation within a less complex user interface that relies on a single demonstration.  

We validate our framework in three simulated and four real-world experiments using a physical 6-DOF robot. It has to be noted that our framework is not limited to a specific set of LfD representations or similarity metrics. However, it has to be noted that each metric favors a specific reproduction feature (e.g., converging to the demonstration vs. preserving shape of the trajectory) which means it is implicitly biased towards a specific representation. To categorize similarity metrics according to their bias towards different reproduction features, we have evaluated 11 metrics for 26 skills for a total of 286 simulated experiments.
